DiffuseKronA: A Parameter Efficient Fine-tuning Method for Personalized Diffusion Models

In the realm of subject-driven text-to-image (T2I) generative models, recent developments like DreamBooth and BLIP-Diffusion have led to impressive results yet encounter limitations due to their intensive fine-tuning demands and substantial parameter requirements. While the low-rank adaptation (LoRA) module within DreamBooth offers a reduction in trainable parameters, it introduces a pronounced sensitivity to hyperparameters, leading to a compromise between parameter efficiency and the quality of T2I personalized image synthesis. Addressing these constraints, we introduce \textbf{\textit{DiffuseKronA}}, a novel Kronecker product-based adaptation module that not only significantly reduces the parameter count by 35\% and 99.947\% compared to LoRA-DreamBooth and the original DreamBooth, respectively, but also enhances the quality of image synthesis. Crucially, \textit{DiffuseKronA} mitigates the issue of hyperparameter sensitivity, delivering consistent high-quality generations across a wide range of hyperparameters, thereby diminishing the necessity for extensive fine-tuning. Furthermore, a more controllable decomposition makes \textit{DiffuseKronA} more interpretable and even can achieve up to a 50\% reduction with results comparable to LoRA-Dreambooth. Evaluated against diverse and complex input images and text prompts, \textit{DiffuseKronA} consistently outperforms existing models, producing diverse images of higher quality with improved fidelity and a more accurate color distribution of objects, all the while upholding exceptional parameter efficiency, thus presenting a substantial advancement in the field of T2I generative modeling. Our project page, consisting of links to the code, and pre-trained checkpoints, is available at https://diffusekrona.github.io/.

==> tex/table.tex <==
\begin{table}[!ht]
    \centering
    \begin{tabular}{c|c|c}
    \toprule
        \textbf{$a_{1}$} & \textbf{$a_{2}$} & \textbf{\# Parameters} \\
        \midrule

        \multirow{7}{*}{2} & 2 & 238799040\\
        & 4 & 119402880 \\
        & 8 & 59708160 \\
        & 16 & 29867520 \\
        & 32 & 14960640\\
        & 64 & 7534080\\
        & 128 & 3874560\\

        \midrule
        \multirow{7}{*}{4} & 2 & 119402880\\
        & 4 & 59708160\\
        & 8 & 29867520\\
        & 16 & 14960640\\
        & 32 & 7534080\\
        & 64 & 3874560\\
        & 128 & 2152320\\

        \midrule
        \multirow{7}{*}{8} & 2 & 59708160\\
        & 4 & 29867520\\
        & 8 & 14960640\\
        & 16 & 7534080\\
        & 32 & 3874560\\
        & 64 & 2152320\\
        & 128 & 1506240\\

        \midrule
        \multirow{7}{*}{16} & 2 & 29867520\\
        & 4 & 14960640\\
        & 8 & 7534080\\
        & 16 & 3874560\\
        & 32 & 2152320\\
        & 64 & 1506240\\
        & 128 & 1613280\\

        \midrule
        \multirow{7}{*}{32} & 2 & 14960640\\
        & 4 & 7534080 \\   
        & 8 & 3874560\\
        & 16 & 2152320\\
        & 32 & 1506240\\
        & 64 & 1613280\\
        & 128 & 2526960\\
        
        \midrule
        \multirow{7}{*}{64} & 2 & 7534080\\
        & 4 & 3874560\\
        & 8 & 2152320\\
        & 16 & 1506240\\
        & 32 & 1613280\\
        & 64 & 2526960\\
        & 128 & 4704120\\

        \midrule
        \multirow{7}{*}{128} & 2 & 3874560\\
         & 4 & 2152320\\
         & 8 &  1506240\\
         & 16 & 1613280\\
         & 32 & 2526960\\
         & 64 & 4704120\\
         & 128 & 9233340\\

         
         
    \bottomrule
    \end{tabular}
    \caption{Effect of size of Kronecker Factors in terms of trainable parameter count}
    \label{tab:param_krona}
\end{table}

\begin{table*}[ht]
  \centering
  \begin{tabular}{c|c}
    \begin{tabular}{ccc}
        \begin{tabular}{c|c|c}
        \toprule
        \textbf{$a_{1}$} & \textbf{$a_{2}$} & \textbf{\# Parameters} \\
        \midrule
        \multirow{7}{*}{1} & 2 & 123456789\\
        & 4 & 123456789\\
        & 8 &  123456789\\
        & 16 & 123456789\\
        & 32 & 123456789\\
        & 64 & 123456789\\
        & 128 & 123456789\\
        \bottomrule
      \end{tabular}
    \end{tabular}
    &
      \begin{tabular}{c|c|c}
        \toprule
        \textbf{$a_{1}$} & \textbf{$a_{2}$} & \textbf{\# Parameters} \\
        \midrule
        \multirow{7}{*}{2} & 2 & 238799040\\
        & 4 & 119402880 \\
        & 8 & 59708160 \\
        & 16 & 29867520 \\
        & 32 & 14960640\\
        & 64 & 7534080\\
        & 128 & 3874560\\
        \bottomrule
      \end{tabular}   
      \\
      \begin{tabular}{c|c|c}
        % \toprule
        \textbf{$a_{1}$} & \textbf{$a_{2}$} & \textbf{\# Parameters} \\
        \midrule
        \multirow{7}{*}{4} & 2 & 119402880\\
        & 4 & 59708160\\
        & 8 & 29867520\\
        & 16 & 14960640\\
        & 32 & 7534080\\
        & 64 & 3874560\\
        & 128 & 2152320\\
        \bottomrule
       \end{tabular}
      &
      \begin{tabular}{c|c|c}
        % \toprule
        \textbf{$a_{1}$} & \textbf{$a_{2}$} & \textbf{\# Parameters} \\
        \midrule
        \multirow{7}{*}{8} & 2 & 59708160\\
        & 4 & 29867520\\
        & 8 & 14960640\\
        & 16 & 7534080\\
        & 32 & 3874560\\
        & 64 & 2152320\\
        & 128 & 1506240\\
        \bottomrule
      \end{tabular}
        \\
      \begin{tabular}{c|c|c}
        % \toprule
        \textbf{$a_{1}$} & \textbf{$a_{2}$} & \textbf{\# Parameters} \\
        \midrule
        \multirow{7}{*}{16} & 2 & 29867520\\
        & 4 & 14960640\\
        & 8 & 7534080\\
        & 16 & 3874560\\
        & 32 & 2152320\\
        & 64 & 1506240\\
        & 128 & 1613280\\
        \bottomrule
      \end{tabular}
      &
      \begin{tabular}{c|c|c}
        % \toprule
        \textbf{$a_{1}$} & \textbf{$a_{2}$} & \textbf{\# Parameters} \\
        \midrule
        \multirow{7}{*}{32} & 2 & 14960640\\
        & 4 & 7534080 \\   
        & 8 & 3874560\\
        & 16 & 2152320\\
        & 32 & 1506240\\
        & 64 & 1613280\\
        & 128 & 2526960\\
        \bottomrule
      \end{tabular}
    \\
      \begin{tabular}{c|c|c}
        % \toprule
        \textbf{$a_{1}$} & \textbf{$a_{2}$} & \textbf{\# Parameters} \\
        \midrule
        \multirow{7}{*}{64} & 2 & 7534080\\
        & 4 & 3874560\\
        & 8 & 2152320\\
        & 16 & 1506240\\
        & 32 & 1613280\\
        & 64 & 2526960\\
        & 128 & 4704120\\
        \bottomrule
      \end{tabular}
      &
      \begin{tabular}{c|c|c}
        % \toprule
        \textbf{$a_{1}$} & \textbf{$a_{2}$} & \textbf{\# Parameters} \\
        \midrule
        \multirow{7}{*}{128} & 2 & 3874560\\
        & 4 & 2152320\\
        & 8 &  1506240\\
        & 16 & 1613280\\
        & 32 & 2526960\\
        & 64 & 4704120\\
        & 128 & 9233340\\
        \bottomrule
      \end{tabular}

  \end{tabular}
  \caption{Effect of size of Kronecker Factors in terms of trainable parameter count}
  \label{tab:param_krona}
\end{table*}
